A portable muon telescope based on small and gas-tight Resistive Plate Chambers

We report on the first steps in the development of a small-size muon telescope based on glass Resistive Plate Chambers with small active area ($16\times 16~{\rm cm}^2$). The long-term goal of this project is to focus on applications of muography where the telescope may have to be operated underground and/or inside small rooms, and in challenging logistic situations. Driving principles in our design are therefore compact size, light weight, gas tightness, and robustness. The first data-taking experiences have been encouraging, and we elaborate on the lessons learnt and future directions for development.

==> aucontribute.tex <==
SW built the set-up, carried out the experiments, and performed the data analysis. AG and ECG conceived of and designed the study. PD set up the software for data acquisition, high-voltage and threshold scans, and assisted the data analysis. AG drafted the manuscript. All authors read and approved the manuscript.

==> dataccess.tex <==
The raw data used to produce the results shown in this article, as well as the ROOT~\cite{root} scripts needed to analyse them, are publicly available and documented at \url{https://github.com/sowuy/Muoscope}. The mechanical drawings of our detectors are available at \url{https://github.com/sowuy/User-Guide}.
